Numerical Analysis of Target Enumeration via Euler Characteristic Integrals

Given a continuous sensor field, we can apply the Euler characteristic integral approach to count the number of targets in the sensor field. If the sensor field is discrete, the Euler integral approach introduces errors into our target count. In this paper, we study the behavior of the Euler integral when applied to discrete sensor fields. Under precise assumptions, we count the number of first- and second-order errors in target count, and discover a formula proportional to much higher order errors. This allows us to derive a point estimator for the number of targets in a discrete sensor field. Finally we derive an asymptotic result, providing insight into how the discrete Euler integral behaves for a large number of targets.

==> Titlepage_backup.tex <==
\large\newlength{\oldparskip}\setlength\oldparskip{\parskip}\parskip=.3in
\thispagestyle{empty} \doublespaced
\begin{center}
\vspace*{\fill} \thetitle

\theauthor


A THESIS

in

Mathematics

\large Presented to the Faculties of the University of
Pennsylvania in Partial
 Fulfillment of the Requirements for the Degree of Master of
 Arts

\large
\theyear
\end{center}


\noindent\makebox[0in][l]{\rule[2ex]{3in}{.3mm}}
Supervisor of Thesis



\noindent\makebox[0in][l]{\rule[2ex]{3in}{.3mm}} Graduate Group
Chairman \vspace*{\fill}

\normalsize\parskip=\oldparskip


